Feasibility Study of Magnetism-based Indoor Positioning Methods in an Incineration Plant

In an incineration plant, remote operation from a centralized control room is now possible, but inspection and cleaning of equipment still require a worker to visit the site. When the plant owner reduces the number of workers due to operation costs, it will be standard for a single worker to visit the site. Therefore, it is necessary to monitor the location of workers in real-time to detect unexpected human accidents quickly. Conventional methods use radio waves, such as Wi-Fi and Bluetooth, but there is little demand for communication equipment in the incineration plant. However, there is not enough demand for communication facilities in the incineration plant. It is too large to bear the cost of installing wireless access points, and Bluetooth Low Energy (BLE) beacons just for positioning. Therefore, we are focusing on magnetism using for indoor positioning method. In addition, the incineration plant has a lot of types of equipment that contains a wide range of magnetized metals, large motors, and generators. We could observe the magnetic peculiarity at each point. Based on these assumptions, we have developed a new indoor positioning method at the incineration plant. This paper describes the development of an indoor positioning system for an incineration plant. And we propose three methods for fingerprinting matching: Point matching, Path matching, and DTW matching. The average positioning errors of these methods are 6.89 m, 0.05 m, and 0.06 m, respectively.

==> subtex/alg2.tex <==
% !TeX root = ../percom2022ws_rei-ok_eng.tex

\begin{algorithm}[b!]
    \caption{\ Path Matching}
    \label{alg:path_matching}
    \begin{algorithmic}
        \renewcommand{\algorithmicrequire}{\textbf{Input:}}
        \renewcommand{\algorithmicensure}{\textbf{Output:}}

        \Require \\
        \begin{itemize}
            \item $RefPaths[\;][\;] = RefPath_1[\;], \dots, RefPath_n[\;]$

            List of path collected at offline phase.
            \item {\small $TarPath[\;] = {\rm tar}(Mv_1, \ Mh_1), \dots, {\rm tar}(Mv_m, \ Mh_m)$}

            List of matching target $(M_v, \ M_h)$.
        \end{itemize}
        \Ensure \\
        \begin{itemize}
            \item $AnsRefPath[\;]$

            Path of estimation result.
            \item $idx$

            How many points in the line should be the starting point?
        \end{itemize}
        \State
    \end{algorithmic}
    \begin{algorithmic}[1]
        \State $minScore \gets 1000000000$ \Comment{Huge number}
        \State $AnsRefPath[\;] \gets RefPaths_1[\;]$
        \State $M \gets {\rm \ length \ of} \ TarPath[\;] $
        \ForAll {$RefPath_j[\;] \in RefPaths[\;][\;]$}
            \State $idx \gets 1$
            \State $L \gets {\rm \ length \ of} \ RefPath_j[\;] $
            \For {$i \gets 1 \ {\rm to} \  L - M$}
                \State $RefPoints[\;] \gets RefPath_j[i \ {\rm to} \ i + M]$
                \State $scores \gets$ Calculate the Euclidean distance between each point in $RefPoints[\;]$ and $TarPath[\;]$.
                \State $score \gets mean(scores)$ \Comment{Calculate the arithmetic mean.}
                \If {$score < minScore$}
                    \State $AnsRefPath[\;] \gets RefPath[\;]$
                    \State $idx \gets i$
                \EndIf
            \EndFor
        \EndFor
        \State \Return $AnsRefPath[\;]$, $idx$
        \end{algorithmic}
\end{algorithm}


==> subtex/alg3.tex <==
% !TeX root = ../percom2022ws_rei-ok_eng.tex

\begin{algorithm}[tb]
    \caption{\ DTW Matching}
    \label{alg:line_dtw_matching}
    \begin{algorithmic}
        \renewcommand{\algorithmicrequire}{\textbf{Input:}}
        \renewcommand{\algorithmicensure}{\textbf{Output:}}

        \Require \\
        \begin{itemize}
            \item $RefPaths[\;][\;] = RefPath_1[\;], \dots, RefPath_n[\;]$

            List of path collected at offline phase.
            \item {\small $TarPath[\;] = {\rm tar}(Mv_1, \ Mh_1), \dots, {\rm tar}(Mv_m, \ Mh_m)$}

            List of matching target $(M_v, \ M_h)$.
        \end{itemize}
        \Ensure \\
        \begin{itemize}
            \item $AnsRefPath[\;]$

            Path of estimation result.
            \item $idx$

            How many points in the line should be the starting point?
        \end{itemize}
        \State
    \end{algorithmic}
    \begin{algorithmic}[1]
        \State $minScore \gets 1000000000$ \Comment{Huge number}
        \State $AnsRefPath[\;] \gets RefPaths_1[\;]$
        \State $M \gets {\rm \ length \ of \ } TarPath[\;]$
        \ForAll {$RefPath_j[\;] \in RefPaths[\;][\;]$}
            \State $idx \gets 1$
            \State $L \gets {\rm \ length \ of} \ RefPath_j[\;] $
            \For {$i \gets 1 \ {\rm to} \  L - M$}
                \State $RefPoints[\;] \gets RefPath_j[i \ {\rm to} \ i + M]$
                \State $scoreDtw \gets$ Calculate the DTW score in $RefPoints[\;]$ and $TarPath[\;]$.
                % \State $score \gets \frac{1}{1 + scoreDtw}$
                \If {$scoreDtw < minScore$}
                    \State $AnsRefPath[\;] \gets RefPath[\;]$
                    \State $idx \gets i$
                \EndIf
            \EndFor
        \EndFor
        \State \Return $AnsRefPath[\;]$, $idx$
        \end{algorithmic}
\end{algorithm}

